"False negative -- that one is going to kill you": Understanding Industry Perspectives of Static Analysis based Security Testing

The demand for automated security analysis techniques, such as static analysis based security testing (SAST) tools continues to increase. To develop SASTs that are effectively leveraged by developers for finding vulnerabilities, researchers and tool designers must understand how developers perceive, select, and use SASTs, what they expect from the tools, whether they know of the limitations of the tools, and how they address those limitations. This paper describes a qualitative study that explores the assumptions, expectations, beliefs, and challenges experienced by developers who use SASTs. We perform in-depth, semi-structured interviews with 20 practitioners who possess a diverse range of software development expertise, as well as a variety of unique security, product, and organizational backgrounds. We identify $17$ key findings that shed light on developer perceptions and desires related to SASTs, and also expose gaps in the status quo - challenging long-held beliefs in SAST design priorities. Finally, we provide concrete future directions for researchers and practitioners rooted in an analysis of our findings.

==> method.tex <==
\section{Methodology}\label{sec:method}



To understand the potentially diverse perspectives of practitioners related to \sasts, we performed a two-phase study, consisting of
$(a)$ a survey (Section~\ref{sec:online-survey}), that helped us develop an initial understanding and guided the $(b)$ in-depth, detailed interviews of practitioners (detailed in Section~\ref{subsec:interview-protocol}).
Figure~\ref{fig:flow-survey-interview} gives an overview of the survey and the interview approach.
We give an overview of the protocols, recruitment strategy, ethical considerations, coding and analysis in this section, and the summary of survey and interview questions in the appendices~\ref{app:survey-questions} and \ref{app:interview-guide} respectively.
Furthermore, the full details of these two phases, including the informed consent forms, survey questionnaire, and the interview guide are available in the online appendix~\cite{online-appendix}.

\input{survey-methodology.tex}
\input{interview-methodology.tex}

==> survey-methodology.tex <==
\section{Survey Protocol}\label{sec:online-survey}
To understand how practitioners perceive security tools, and whether security is prioritized by individuals and organizations similarly, we prepared an online survey questionnaire (abridged questionnaire in Appendix~\ref{app:survey-questions}) and drafted a research protocol.
We piloted the initial survey with five participants. Three of the participants were graduate students, and the rest had doctoral degrees. All pilots were from computer science background, with additional experience in software engineering and/or security.
By incorporating their feedback, we improved the survey by modifications and additional descriptions as necessary.
Our final survey protocol received the approval of our Institutional Review Boards (IRBs).
The experimental protocol of both our survey and interviews included a consent form which emphasized that the data of the participants will remain confidential and de-identified.
Furthermore, a participant could optionally submit their email address to have the chance of winning one of two $\$50.00$ gift cards or the equivalent value in local currency vouchers. The winners would be chosen from qualified participants who completed the survey and provided valid responses in the survey.



\subsection{Survey Recruitment}
To diversify our recruitment approach in terms of experience, culture and industry contexts, we leveraged multiple recruitment channels.
We sent invitation emails describing the goal of the survey (\ie in order to learn about their professional experiences and opinions about \sasts) to the following groups of people:

\myparagraphnew{Professional Networks}: We relied on Snowball-sampling~\cite{SnowballSamplinggoodman1961a} to recruit from our professional networks across borders.
We sent survey invitation emails that similarly contained research goal. Furthermore, we requested them to forward the invitation to their relevant colleagues who might be potentially interested.
Through this approach, we received $21$ complete and valid survey responses.

\myparagraphnew{Open Source Software (OSS) Developers}: We emailed OSS developers who had interacted with \sasts via CI/CD actions, such as GitHub Workflows, in open-source repositories that $(a)$ had at least one star or watcher, $(b)$ were not a fork, and $(c)$ used one of the top ten programming languages in GitHub between Aug - Sept 2021. We collected publicly available email addresses only, and explicitly stated our recruitment procedure in our initial contact, which is common in other recent studies (\eg \cite{EBW22}).
\\\textit{\underline{Ethical Considerations:}}
We considered several \textit{potential trade-offs} that factored into this recruitment strategy, in addition to following the guidance provided by our IRB:
$(a)$ It is \textit{difficult} to recruit practitioners across borders who have the relevant experience, \ie configured and used automated security analysis tools,
$(b)$ we were collecting publicly available information and not amplifying the public visibility of the participants email address or other information, and
$(c)$ we carefully considered the Menlo Report's ethical guidelines on Information and Communication Technology Research from the Dept. of Homeland Security~\cite{KD12,DKB13}.
Specifically based on these guidelines, the only potential \textit{harm} to an invited person would be receiving one unsolicited email, whereas the benefit of this research is potentially helping create more secure software, for everyone, by understanding the needs and challenges of practitioners related to security analysis techniques.
In the end, we contacted $1,918$ potential participants using via email exactly once and received $18$ complete and valid survey responses.




\subsection{Online Survey and Data Analysis}
Our survey (Appendix~\ref{app:survey-questions}) consisted of Likert Scale based questions, with optional, open-ended response to clarify their selected choice(s).
Our analysis prioritized the text-based responses since these provided additional context for the selected choice(s) in Likert scale.
One of the authors open-coded the responses for analysis.
The responses of the survey guided our Interview protocol, which we describe next.

